Danish Foundation Models

Large language models, sometimes referred to as foundation models, have transformed multiple fields of research. However, smaller languages risk falling behind due to high training costs and small incentives for large companies to train these models. To combat this, the Danish Foundation Models project seeks to provide and maintain open, well-documented, and high-quality foundation models for the Danish language. This is achieved through broad cooperation with public and private institutions, to ensure high data quality and applicability of the trained models. We present the motivation of the project, the current status, and future perspectives.

==> tables/table1.tex <==
\begin{table*}[h]
\centering
\caption{A representative sample of different foundation model categories used for Danish: structured learning (e.g. encoders), generative models (e.g. decoders), search and ranking models (embeddings), and speech. Languages are denoted using a flag and multilingual is denoted with \emoji{globe-with-meridians}.
}
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}[t]{lcccclc}
\toprule
 & Model  & Code & Model  & Data  & Language & Validated\\
  & weights & Available  & card & sheet &   & for Danish\\
\midrule
\multicolumn{7}{l}{\textbf{Text}} \\
\multicolumn{7}{l}{\textit{Structured learning}} \\
\hspace{1em} \textbf{dfm-encoder-large-v1} (ours) & \greenchecknospace & \greenchecknospace & \greenchecknospace & \greenchecknospace & \emoji{flag-denmark}
 & \greenchecknospace \\
\hspace{1em} nb-bert-large & \greenchecknospace & \greenchecknospace & \greycrossnospace & \greycrossnospace & \emoji{flag-norway} (\emoji{flag-denmark} \emoji{flag-sweden}) & \greenchecknospace \\
\hspace{1em} XLM-Roberta & \greenchecknospace & \greenchecknospace & \greycrossnospace & \greycrossnospace & \emoji{globe-with-meridians} & \greenchecknospace \\
\multicolumn{7}{l}{\textit{Generative models}} \\
\hspace{1em} GPT-4 & \greycrossnospace & \greycrossnospace & \greycrossnospace & \greycrossnospace & \emoji{flag-united-states} (\emoji{globe-with-meridians}) & \textcolor{white}{*}\greycrossnospace*  \\
\hspace{1em} DanskGPT & \greycrossnospace & \greycrossnospace & \greycrossnospace & \greycrossnospace & \emoji{flag-denmark} & \textcolor{white}{*}\greycrossnospace* \\
\hspace{1em} DanT5 & \greycrossnospace & \greycrossnospace & \greycrossnospace & \greycrossnospace & \emoji{flag-denmark} & \greycrossnospace \\
\hspace{1em} Llama-v2 & \greenchecknospace & \greycrossnospace & \greenchecknospace & \greycrossnospace & \emoji{flag-united-states} & \textcolor{white}{*}\greycrossnospace*  \\
\multicolumn{7}{l}{\textit{Embeddings}} \\
\hspace{1em} text-embedding-ada-2 & \greycrossnospace & \greycrossnospace & \greycrossnospace & \greycrossnospace & \emoji{flag-united-states} (\emoji{globe-with-meridians}) & \textcolor{white}{*}\greenchecknospace* \\
\hspace{1em} MiniLM-L12-v2$^1$& \greenchecknospace & \greenchecknospace & \greycrossnospace & \greenchecknospace & \emoji{globe-with-meridians} & \greenchecknospace \\
\multicolumn{7}{l}{\textbf{Speech}} \\
\multicolumn{7}{l}{\textit{Structured learning}} \\
\hspace{1em} \textbf{dfm-xls-r-300m} (ours) & \greenchecknospace & \greenchecknospace & \greenchecknospace & \greenchecknospace & \emoji{flag-denmark} & \textcolor{white}{*}\greenchecknospace$^\dagger$ \\
\hspace{1em} wav2vec2-base-da & \greenchecknospace & \greenchecknospace & \greycrossnospace & \greycrossnospace & \emoji{flag-denmark} & \textcolor{white}{*}\greenchecknospace$^\dagger$ \\
\bottomrule
\multicolumn{7}{l}{\footnotesize $^1$: \texttt{paraphrase-multilingual-MiniLM-L12-v2}} \\
\multicolumn{7}{l}{\footnotesize *: Proper validation is not possible as the training data is not known (test data might be included).} \\
\multicolumn{7}{l}{\footnotesize $^\dagger$: Finetuned models are validated for Danish ASR, but  there are no existing benchmarks for Danish.} 

\end{tabular}
\end{adjustbox}
\end{table*}
